B-GAP: Behavior-Rich Simulation and Navigation for Autonomous Driving

We address the problem of ego-vehicle navigation in dense simulated traffic environments populated by road agents with varying driver behaviors. Navigation in such environments is challenging due to unpredictability in agents' actions caused by their heterogeneous behaviors. We present a new simulation technique consisting of enriching existing traffic simulators with behavior-rich trajectories corresponding to varying levels of aggressiveness. We generate these trajectories with the help of a driver behavior modeling algorithm. We then use the enriched simulator to train a deep reinforcement learning (DRL) policy that consists of a set of high-level vehicle control commands and use this policy at test time to perform local navigation in dense traffic. Our policy implicitly models the interactions between traffic agents and computes safe trajectories for the ego-vehicle accounting for aggressive driver maneuvers such as overtaking, over-speeding, weaving, and sudden lane changes. Our enhanced behavior-rich simulator can be used for generating datasets that consist of trajectories corresponding to diverse driver behaviors and traffic densities, and our behavior-based navigation scheme can be combined with state-of-the-art navigation algorithms.

==> Tables/crashes.tex <==
\begin{table}[t]
\caption{A comparison of the number of crashes as measured in a frequency over $100$ episodes at test time for different traffic densities (number of vehicles) and varying driving behaviors (Aggressiveness) between the policy generated by our Behavior-Guided simulator (\textit{bottom}) and the policy generated by the default simulator (\textit{top}). Conservative traffic corresponds to fully conservative agents, mixed traffic corresponds to $50\%$ aggressive agents and $50\%$ conservative agents, while aggressive traffic corresponds to $100\%$ aggressive agents. The behavior-guided policy significantly reduces the number of collisions for a diverse range of driving behaviors both in sparse and dense driving scenarios.}
\centering
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc} 
\toprule
\multicolumn{4}{c}{\textbf{Default Policy}}\\
\midrule
\# vehicles & Conservative & Mixed  & Aggressive  \\
$n$ & \multicolumn{3}{c}{\textit{Number of crashes}} \\
\midrule
$5$ & $21$ & $31$ & $11$ \\
$40$ & $65$ & $70$ & $30$ \\
\midrule
\multicolumn{4}{c}{\textbf{Behavior-Guided Policy}}\\
\midrule
\# vehicles & Conservative & Mixed  & Aggressive  \\

$n$ & \multicolumn{3}{c}{\textit{Number of crashes}} \\
\midrule
$5$ & \textbf{5} & \textbf{14} & \textbf{3}\\
$40$ & \textbf{27} & \textbf{36} & \textbf{4}\\
\bottomrule
\end{tabular}
% }
\label{tab: crashes}
\vspace{-10pt}
\end{table}

==> Tables/evaluation.tex <==
\begin{table*}[t]
\caption{ We measure the average speed (Avg. Spd.) and the number of lane changes (\#LC) for the ego-vehicle when it is navigating in the (left) default simulator (without any varying behaviors), interacting with conservative agents only, interacting with a combination of conservative and aggressive traffic-agents, and interacting with aggressive agents only. We vary the number of traffic agents from sparse ($n=5$) to dense ($n=40$). We observe that Avg. Spd. of ego-vehicle is lower in conservative environments because the ego-vehicle is navigating among slow-moving traffic. Further, \#LC is higher in conservative environments as the ego-vehicle attempts to pass the slow-moving vehicles. The default simulator does not distinguish between different behaviors because the Avg. Spd. is approximately the average of the two behaviors.}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccc} 
\toprule
\multicolumn{7}{c}{\textbf{Default Policy}}\\
\midrule
Number of vehicles & \multicolumn{2}{c}{Conservative Traffic} & \multicolumn{2}{c}{Mixed Traffic} &\multicolumn{2}{c}{Aggressive Traffic} \\
 $n$ & \textit{Avg. Spd. (m/s)} & \textit{\#LC} & \textit{Avg. Spd. (m/s)} & \textit{\#LC} & \textit{Avg. Spd. (m/s)} & \textit{\#LC}  \\
\midrule
$5$ & $26.04$ & $10.26$ & $26.25$ & $7.89$ & $26.50$ & $7.21$\\
$40$ & $18.57$ & $5.42$ & $18.70$ & $4.83$ & $19.15$ & $4.41$\\
\midrule
\multicolumn{7}{c}{\textbf{Behavior-Guided Policy}}\\
\midrule
Number of vehicles & \multicolumn{2}{c}{Conservative Traffic} & \multicolumn{2}{c}{Mixed Traffic} &\multicolumn{2}{c}{Aggressive Traffic} \\
 $n$ & \textit{Avg. Spd. (m/s)} & \textit{\#LC} & \textit{Avg. Spd. (m/s)} & \textit{\#LC} & \textit{Avg. Spd. (m/s)} & \textit{\#LC}  \\
 \midrule
 $5$ & $25.05$ & $4.86$ & $27.83$ & $3.82$ & $28.65$ & $3.27$\\
$40$ & $17.77$ & $10.61$ & $20.13$ & $9.49$ & $25.99$ & $3.73$\\
\bottomrule
\end{tabular}
% }
\label{tab: evaluation}
\vspace{-10pt}
\end{table*}

==> algorithms/algo1.tex <==
\begin{algorithm}[t]
    \SetKwInOut{Input}{Initialize}
    \SetKwInOut{Output}{Output}
\SetKwComment{Comment}{$\triangleright$\ }{}
\SetAlgoLined
\Input{Set random simulation parameters $\Xi_0 = \{ T, s_0, a, b, p, \Delta a_{th}, b_{safe} \}$.}
\Output{Final simulation parameters for generating aggressive behaviors.}
\While{not converged}{ 
// Generate trajectories from the current params //\\
$     \zeta^i_c[t] = \frac{N-1}{\Tstrutfrac \sum_{v_j\in \mathcal{V}(t)\setminus \{v_i\}} \mc{D}_t(v_i,v_j)}$ \\ 
$    \zeta^i_d[t] = \bigl | \{ v_j \in \mc{N}_i(t) \} \bigr | + \zeta^i_d[t-1], (v_i,v_j) \not\in \mc{E(\tau)}, \tau = 0, \ldots, t-1$ \\
% $         \zeta^i_e[t] = \frac{1}{\lambda} \sum_{v_j \in \mc{\mc{N}_i}(t)}A_t(v_i,v_j)  \zeta^j_e[t] $\\
$t \gets t+1$ \\
// Use CMetric to quantify the aggressiveness //\\
$\beta = \argmin_\beta \Vts{\zeta - M\beta}$\\
$\zeta(t) = \beta_0 + \beta_1 t + \beta_2t^2$\\
// Adjust parameters //\\
% Form $\cm$ using Definition~\ref{def: cmetric}\\
\For{$k=0,1,2$}{
$\textrm{SLE}_k(t) = \abs*{\frac{\partial \zeta(t)}{\partial t}}$\\
$\textrm{SIE}_k(t) = \abs*{\frac{\partial^2 \zeta(t)}{\partial t^2}}$
}
}

\caption{Our algorithms for generating longitudinal and lateral aggressive driving behaviors for our simulator.}
\label{alg: main}
\vspace{-3pt}
\end{algorithm}


